Mesoscopic approach to minority games in herd regime

We study minority games in efficient regime. By incorporating the utility function and aggregating agents with similar strategies we develop an effective mesoscale notion of state of the game. Using this approach, the game can be represented as a Markov process with substantially reduced number of states with explicitly computable probabilities. For any payoff, the finiteness of the number of states is proved. Interesting features of an extensive random variable, called aggregated demand, viz. its strong inhomogeneity and presence of patterns in time, can be easily interpreted. Using Markov theory and quenched disorder approach, we can explain important macroscopic characteristics of the game: behavior of variance per capita and predictability of the aggregated demand. We prove that in case of linear payoff many attractors in the state space are possible.

==> conclusions_v2.tex <==
\section{Conclusions}
%\addcontentsline{toc}{chapter}{Conclusion}
%
In this paper we proposed a consistent, reductionist scheme explaining phenomenology of minority games in the efficient regime. In this mode the size of strategy space is much smaller than the number of strategies used by agents and the population as a whole can access complete information about the game.

Our discussion begun with the phenomenology. We considered a number of macroscopic random variables, or their moments, characterizing the game and being particularly important for applications, such as the aggregated demand, demand's variance \textit{per capita} and decision's or demand's predictabilities. We studied these variables as functions of the control parameters, e.g. the ratio of the total number of agents to the number of all possible winning histories, as well as their time evolution. Among interesting features we found that predictabilities may, or may not, be sensitive to the form of the payoff function, depending on how the predictabilities are actually defined: using winning decisions only or the overall demand.

Deeper insight into the mechanism of these behaviors was possible by performing coarse-graining and aggregation of some internal degrees of freedom of the game, thus defining an intermediate level of description, called mesoscopic.  At such mesoscopic level, fractions of agents using same strategies are treated as separate entities. Using this method, in the efficient regime when $NS\gg 2^P$, we also managed to represent the game as a Markov process with the finite number of states.

In case where the Markov representation is known, two methodologies were proposed to explain our observations. First, in the simplified case, the quenched disorder was neglected, i.e. fractions were assumed to be equal size. In this case, however, not all observations are properly explained. Behavior of predictability required extended methodology where the quenched disorder was used. Two payoffs, the steplike and linear, were separately analyzed. We showed that in case of the steplike payoff, the stochastic and deterministic transitions were possible, whereas for the linear payoff, all transitions were deterministic.

We argued that the Markov process representation of the game completely defines and explains the dynamics of the game in the stationary regime, and allows for the calculation of state occupancies. If the transition probabilities in the Markov chain are known, the phenomenology also becomes understandable. For example, the Markov representation provides an explanation of the
periodicity and preferred levels of the aggregate demand $A(t)$. In practical terms, this approach is tough for $m>1$ due to the large number of states but the whole reasoning remains valid in general. We failed to find any relation between the memory length $m$ and the total number of states.

Neither the simplified concept of state nor the Markov process description seem to be correct if the initial preference was given to any strategy. The definition of the stability was introduced in Sec.~\ref{sec:stability}, in order to better understand asymmetries observed for aggregated variables. The stability mechanism appeared to be sensitive to the payoff function. In case the steplike payoff was considered, then the frequency of opposite signs of $A$ after any $\mu$ had to be preserved. In case of the linear payoff, the negative and positive values of A had to compensate mutually. As a result, depending on the payoff, both the $H_a$ and $H_A$ were equal to zero in the herd regime.

Differences between systems with equal-size fractions and those with unequal-size fractions were more likely for larger numbers of agents. This was particularly reflected in distortions of: (i) the transition probabilities, in case of the steplike payoff, and (ii) attractors, in case of the linear payoff. In order to quantify this distortion, the measure of distance between two Markov processes was introduced.

We studied games with the full, maximal strategy space. Some authors, e.g. in Refs.~\cite{challet97PhysicaA246,li00PhysicaA284}, reduced the strategy space and reproduced many features of the full MG, e.g. behavior of variance per capita. The drawback of their method is that it reduces the number of states in the Markov-chain description of the game and significantly affects its time evolution. The Markov representation is oversimplified by such reduction.

Some observables for the proportional payoff were explained without using the Markov process. For example, there was an observation of distinct peaks of the aggregated demand, exhibiting height equal to a half of the population, assuming $S = 2$. We showed that in the herd regime, there
always exists a history $\mu_C$ for which the fraction $1-\frac{1}{2^{S}}$ of agents reacts identically and this is seen in the peak $A(t)=N(1-\frac{1}{2^{S-1}})$. Apart from using the Markov chain technique, we found another, simpler one, where only two classes of strategies were used instead of all $2^P$ classes. This technique is not limited to the case $N S \gg 2^P$ but works in the whole herd regime. This approach was also successfully exploited in our analysis of the multi-market minority game~\cite{wawrzyniak09ACS12No4and5}.

Considering further research, it could be a significant achievement if a single, closed-form equation were found for the entire parameter region of the MG. So far, in literature, such equations have indeed been found in the crowded and random regions separately. But a unified description of the entire range of parameters is still lacking.















